AlignBot: Aligning VLM-powered Customized Task Planning with User Reminders Through Fine-Tuning for Household Robots

This paper presents AlignBot, a novel framework designed to optimize VLM-powered customized task planning for household robots by effectively aligning with user reminders. In domestic settings, aligning task planning with user reminders poses significant challenges due to the limited quantity, diversity, and multimodal nature of the reminders. To address these challenges, AlignBot employs a fine-tuned LLaVA-7B model, functioning as an adapter for GPT-4o. This adapter model internalizes diverse forms of user reminders-such as personalized preferences, corrective guidance, and contextual assistance-into structured instruction-formatted cues that prompt GPT-4o in generating customized task plans. Additionally, AlignBot integrates a dynamic retrieval mechanism that selects task-relevant historical successes as prompts for GPT-4o, further enhancing task planning accuracy. To validate the effectiveness of AlignBot, experiments are conducted in real-world household environments, which are constructed within the laboratory to replicate typical household settings. A multimodal dataset with over 1,500 entries derived from volunteer reminders is used for training and evaluation. The results demonstrate that AlignBot significantly improves customized task planning, outperforming existing LLM- and VLM-powered planners by interpreting and aligning with user reminders, achieving 86.8% success rate compared to the vanilla GPT-4o baseline at 21.6%, reflecting a 65% improvement and over four times greater effectiveness. Supplementary materials are available at: https://yding25.com/AlignBot/

==> temp <==
% \section{Framework}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AdaBot is a closed-loop system designed to deliver a high successful rate, real-time, and personalized embodied large model with continuous iterative learning. The system integrates a multimodal language model (Instruction-LLaVA), a multimodality memory base with continuous iteration and reranking capabilities, a high-reasoning model for action planning, an advanced image post-processor for enhancing spatial information, and the high-success-rate motion model ABC. The components achieve efficiently processing complex user instructions and ultimately driving robotic arms to execute tasks.

% The cornerstone of the AdaBot system is Instruction-LLaVA, a personalized language model meticulously fine-tuned based on the LLaVA architecture. This model serves as the primary source of input instructions for the action planning model, enhancing its capabilities in logical reasoning and action planning. GPT-4o represents the current state-of-the-art in multimodal models, employing an end-to-end Transformer architecture. It has achieved top ability in instruction execution, logical reasoning, and motion planning efficiency. Within the AdaBot system, GPT-4o functions as the core planning model for robotic arm operations, demonstrating superior planning success in tasks exemplified by [Robot Control Sample].

% Nevertheless, empirical evaluations reveal that GPT-4o exhibits limitations in handling personalized preference reasoning, integrating historical feedback, and iteratively refining its reasoning based on feedback. Specifically, GPT-4o shows a reduced success rate in task planning when confronted with complex user instructions, and it struggles to adapt its planning process following errors due to insufficient consideration of personalized information.

% To address these challenges, we leveraged the in-context learning capabilities of large language models and introduced a LLaVA-enhanced system designed to augment overall performance. The development of Instruction-LLaVA involved the fine-tuning of the LLaVA model, incorporating model fine-tuning, multimodal memory data integration, image augmentation, and reasoning enhancement. This customization tailored the Instruction-LLaVA model specifically for action planning model.

% Furthermore, to enhance the action planning model’s ability to extract information from images, we implemented an advanced image post-processor. This approach enhances the spatial understanding of 2D images by generating corresponding 3D information, depth maps, and point clouds. By enriching the spatial information in images, the action planning model can more accurately determine the position and state of objects, thereby improving the precision of motion planning decisions.

% Concurrently, the iterative development process facilitated the creation of an efficient multimodal memory base, which archives scene observations and feedback-correction data from past interactions. This memory base plays a pivotal role in augmenting the action planning model’s ability to comprehend and synthesize user preferences, while also assisting in the continuous fine-tuning of Instruction-LLaVA, thereby enhancing the precision of the system's instructional outputs.

% The feedback-driven iterative loop fosters continuous learning and optimization within the system. As a result, the model progressively refines its ability to interpret user needs and generate increasingly accurate plans. This dynamic refinement process not only enhances the precision of robotic actions but also significantly improves the system's responsiveness and reliability in managing complex tasks, culminating in a more intuitive and satisfying user experience.

% The comprehensive architecture of AdaBot markedly advances the overall performance of robotic systems, establishing new benchmarks in execution success rates and alignment with personalized user preferences.

% A key component of the system is the Instruction-LLaVA, a personalized adaptive language model based on the LLaVA architecture. The Instruction-LLaVA finetuned by user feedback from the memory base and provides complete instructions to action planning models. This ensures that the motion plan generated by action planning model meets the user's expectations. These instructions include the user's personalized preferences and planning guidance. Every time a plan is generated, its plausibility and executability are evaluated by the user. If adjustments are needed, users  provide feedback to correct action planning model.

% To address these challenges, we leveraged the in-context learning capabilities of large language models and introduced a LLaVA-enhanced system designed to augment overall performance. The development of Instruction-LLaVA involved the fine-tuning of the LLaVA model, incorporating model fine-tuning, multimodal memory data integration, image augmentation, and reasoning enhancement. This customization tailored the Instruction-LLaVA model specifically for action planning model.

% Concurrently, the iterative development process facilitated the creation of an efficient multimodal memory base, which archives scene observations and feedback-correction data from past interactions. This memory base plays a pivotal role in augmenting the action planning model’s ability to comprehend and synthesize user preferences, while also assisting in the continuous fine-tuning of Instruction-LLaVA, thereby enhancing the precision of the system's instructional outputs.

% The feedback-driven iterative loop fosters continuous learning and optimization within the system. As a result, the model progressively refines its ability to interpret user needs and generate increasingly accurate plans. This dynamic refinement process not only enhances the precision of robotic actions but also significantly improves the system's responsiveness and reliability in managing complex tasks, culminating in a more intuitive and satisfying user experience.


% \subsection{Memory base construction}
The Memory base in the AdaBot model is an essential component that enhances the system's performance and adaptability. It captures images of the scene when a task is performed and stores them along with text descriptions. These descriptions includes noting the important items, their statuses, and the spatial relationships between them. By combining visual and textual information, the memory base provides detailed context to help GPT-4o understand and replicate successful strategies, improving its accuracy in motion planning.

In addition to the scene description, the memory base  also store the user portraits, the motion plan generated for that specific instance, and the corresponding user feedback. For motion planning, the system normalizes GPT-4o's output into Python code. This approach is particularly beneficial as it breaks down the entire motion plan into discrete, quantifiable skills, making it easier for the robot to execute complex operations with precision.
\begin{verbatim}
def Put_the_apple_in_fridge(): 
    find("fridge") 
    walktowards("fridge") 
    open("fridge") 
    find("red apple on the counter") 
    walktowards("red apple on the counter") 
    grab("red apple on the counter") 
    putin("red apple", "fridge") 
    close("fridge") 
    done()
\end{verbatim}

When the user confirms that a motion plan is executable, the Memory base also records this final plan. We have found that these final plans are highly beneficial for GPT-4o when generating motion plans for similar tasks in the future. To leverage this, we designed a simple algorithm: when the user requests a previously issued task, the Memory base sub-library, which consists of final plans, provides the highest-rated final plan to GPT-4o. The rating is based on the success rate of past planning efforts by GPT-4o.

Initially, when all final plans have the same score, five plans are randomly selected and provided to GPT-4o. The user then observes the plans generated by GPT-4o based on this information. If the generated plan is successful, points are added to the corresponding final plans; if unsuccessful, points are deducted. Through multiple iterations, a gap in the scores of final plans  emerge, making the most valuable final plans stand out. This process ensures that the system continuously improves and refines its motion planning capabilities by prioritizing the most effective strategies.

The Instruction-LLaVA is a critical component of the AdaBot system, acting as a personalized language model that is built upon the LLaVA architecture. LLaVA is a model architecture designed to integrate language and visual information, enabling the system to process and understand multimodal inputs effectively. 

In the AdaBot system, the Instruction-LLaVA leverages the LLaVA architecture to interpret user feedback, understand scene dynamics, and provide granular instructions to GPT-4o. The training process for this model involves fine-tuning on a diverse dataset that includes both text and visual information, reflecting the association between tasks, user feedback, and task scenarios. The dataset covers a wide range of scenarios where a robot needs to interpret visual inputs and execute instructions based on those inputs.

% 在训练LLaVA模型的过程中，用户ID、任务目标和用户反馈被结合起来形成问答对，结合场景信息的图片用于训练模型。LLaVA模型学习将视觉输入（如环境图像）与相应的文本描述、目标结合，从而使LLaVA能够掌握用户偏好信息，并使得LLaVA生成的指令与用户的期望紧密对齐。此外，通过训练模型的图像感知能力，提高了其准确识别场景和图像中物品状态的能力。这种综合训练方法使LLaVA模型能够有效解读视觉和输入的文本信息，从而生成更精确、与用户需求一致的指令。

During the fine-tuning of the LLaVA model, user IDs, task objectives, and user feedback are combined to form question-answer pairs, while scenario-specific images are used to train the model. The LLaVA model learns to associate visual inputs, such as scenarios images, with corresponding text descriptions and goals. This process enables Instruction-LLaVA to understand user preferences, ensuring that the instructions generated align closely with user expectations. Additionally, the model's image perception capabilities are enhanced, allowing it to accurately recognize objects and their states within images. This integrated training approach equips the LLaVA model to effectively interpret both visual and textual inputs, leading to the generation of more precise instructions that meet user needs.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To ensure the Instruction-LLaVA effectively interprets visual and contextual information, the model was fine-tuned using the Low-Rank Adaptation (LoRA) method\cite{hu2022lora}. 
We fine-tuned the LLaVA1.5-7B-Chat model with the following key hyperparameters:

\begin{itemize}
\item \textbf{Backbone Model:} LLaVA 1.5-7B-Chat.
\item \textbf{Learning Rate:} 5e-5.
\item \textbf{Epochs:} 40 epochs.
\item \textbf{Gradient Normalization:} 1.0.
\item \textbf{Data Type:} BF16.
\item \textbf{Max Input Length:} 1024 tokens.
\item \textbf{Batch Size:} A batch size of 8, with gradient accumulation set to 4, resulting in an effective batch size of 32 for each weight update.
\item \textbf{Learning Rate Scheduler:} Cosine learning rate scheduler.
\item \textbf{LoRA Rank:} 32.
\item \textbf{LoRA Alpha:} 64.
\item \textbf{LoRA Dropout:} 0.05.
\item \textbf{LoRA Module:} All linear layers.

\end{itemize}

The training was conducted using the PEFT framework, which facilitated the efficient fine-tuning of the LLaVA model for the specific requirements of the AdaBot system\cite{peft}.
During the training process, various prompts were constructed by combining visual inputs with task-specific instructions and user feedback. For example:

\begin{itemize}
\item Visual Input: An image of a kitchen with scattered utensils and snacks.
\item Task Objective: "Organize the kitchen by placing utensils in their designated places."
\item User Feedback: "Ensure that all knives are placed in the drawer."

\item Instruction-LLaVA Output: "xxx"\cpa{Add Example Here}
\end{itemize}

The model is trained to generate appropriate actions based on this data, such as identifying tools in images and providing step-by-step instructions, or pointing other models to areas that need more attention.

During the fine-tuning of the LLaVA model using the LoRA method, the optimization process is guided by the Cross-Entropy Loss function. The loss function used is defined as:

\[
\mathcal{L} = - \frac{1}{N} \sum_{i=1}^{N} \sum_{j=1}^{M} y_{i,j} \log(\hat{y}_{i,j})
\]

Where:

\begin{itemize}
    \item \( \mathcal{L} \) is the overall loss value that needs to be minimized.
    \item \( N \) represents the batch size, i.e., the number of samples in a batch.
    \item \( M \) denotes the length of the output sequence (i.e., the number of tokens in the output).
    \item \( y_{i,j} \) is the ground truth label for the \( i \)-th sample at the \( j \)-th position.
    \item \( \hat{y}_{i,j} \) is the predicted probability distribution of the model for the \( i \)-th sample at the \( j \)-th position.
\end{itemize}

During the fine-tuning process, this loss function helps in adjusting the weights of the model, including the additional low-rank matrices introduced by the LoRA method. These low-rank matrices are integrated into the linear layers of the model, allowing the model to adapt to new tasks with fewer parameters while still maintaining performance.

When the dataset is small, the training strategy needs to be adjusted accordingly. For instance, with only 3 or 4 samples per task, we increase the number of epochs to 60 to enhance the model's memory ability. As the dataset grows, we gradually reduce the number of epochs, eventually stabilizing at 40 to ensure the model maintains strong reasoning abilities.

This process ensures that the instructions it generates align closely with the user's expectations. The model’s image perception capabilities undergo specialized training to enhance its ability to accurately identify scenes and the status of items within those images. This comprehensive training approach equips the LLaVA model to effectively interpret visual and contextual information, resulting in more precise and user-aligned instructions.

\subsubsection{Specification of Instruction}
During experiments, we observed that planning errors in GPT-4o were often due to insufficient information or incorrect target identification. To enhance the success rate of GPT-4o's planning, we categorized human feedback from failed attempts into the following three types:

\begin{itemize}
    \item \textbf{Personalized cues:} These include user-specific preferences or specific rules for object placement.
    \item \textbf{Scene cues:} These cues provide detailed information about the items present and their current status in the scene.
    \item \textbf{Robot Action Sequence cues:} These outline the sequence of actions the robot should perform.
\end{itemize}

To ensure that the instructions generated by Instruction-LLaVA are effectively utilized by GPT-4o, we established a series of specifications aimed at standardizing and constraining these instructions. The focus is on improving clarity, relevance, and execution accuracy. Specifically, the instructions must adhere to the following standards:

\begin{itemize}
    \item \textbf{Conciseness and Logical Sequence:} Instructions should be clear and direct, avoiding complex sentence structures and minimizing ambiguity. Each action should be presented in a step-by-step format, ensuring a natural progression.
    \item \textbf{Contextual Relevance:} The instructions should incorporate essential scene details and user preferences, ensuring that GPT-4o has all necessary information for informed decision-making.
    \item \textbf{Terminological Consistency:} Standardized language should be used throughout the instructions, employing terms that are familiar and unambiguous to GPT-4o.
    \item \textbf{Fallback Options:} Instructions should include contingency plans to handle potential errors or unforeseen scenarios, ensuring that GPT-4o can continue executing tasks even when deviations from the expected process occur.
\end{itemize}

An example of an instruction set generated by Instruction-LLaVA, designed to guide GPT-4o, is as follows:


This approach ensures that the instructions generated by Instruction-LLaVA are aligned with user expectations and are executed accurately by GPT-4o, thereby improving the overall success rate of task completion.


\subsubsection{Enhancing Recognition}

Although LLaVA possesses powerful multi-modal combined analysis capabilities, its image recognition abilities still have room for improvement. Enabling Language and Multimodal Models (LMMs) to capture fine-grained visual details remains a significant challenge.

When generating instructions for GPT-4o, the Instruction-LLaVA requires two key abilities:
\begin{itemize}
\item Target Identification: Accurately identifying the items present in an image. This affects GPT-4o action planning objects.
\item Item Status Identification: Determining the current state or condition of the items in the image. The state of objects can significantly impact the actions that need to be taken.
\end{itemize}
A straightforward approach to achieving this is by creating visual recognition question-and-answer templates specifically designed for the training images.

To enhance the Instruction-LLaVA's capabilities, we developed two specialized datasets:

1. A recognition dataset focused on identifying items within a scene. This dataset is designed to improve Instruction-LLaVA's ability to accurately identify various objects in current environments. For each object, the dataset includes 3-4 positive samples where the object is positioned differently within the scene, with images taken from varying distances and angles. Additionally, it contains 2-3 negative samples where the object is obscured or partially hidden. By including both positive and negative samples, this dataset provides a comprehensive training set that helps the model develop a nuanced understanding of object recognition, thereby enhancing its accuracy and reliability across different scenarios.

2. A dataset designed to capture items in various states. For example, recognizing the open or closed status of a refrigerator door. Each state of an item is represented by approximately 4-5 images, providing a diverse set of visual examples that highlight the variations within each state. These images are then paired with recognition question-answer templates, which guide the model during training to associate specific visual cues with the correct state identification.The inclusion of multiple images for each state ensures that the model is exposed to a range of scenarios, including different angles, lighting conditions, and partial obstructions, making it more robust in real-world applications.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We employed the Low-Rank Adaptation (LoRA) method to fine-tune the LLaVA1.5-7B-Chat model, enabling it to effectively interpret both visual and contextual information. 
LoRA introduces low-rank matrices, significantly reducing the number of trainable parameters, which allows for more efficient fine-tuning on specific tasks.
In our case, we froze the GPT parameters and focused solely on fine-tuning LLaVA, as this retained LLaVA's strengths in visual recognition and task understanding while improving its performance in semantic grounding and cue generation tasks.
In terms of multi-task training, we initially explored joint training under a single loss function but found that it introduced negative interference between tasks, especially because the goals of semantic grounding and cue generation are distinct. 
As a result, we adopted a sequential training strategy, first fine-tuning LLaVA on semantic grounding tasks and then on cue generation.
This phased approach allows the model to use the knowledge from the semantic grounding phase—such as object and state recognition—as prior knowledge, improving its ability to generate accurate cues aligned with user feedback.
Training Process and Hyperparameters: A critical focus of our fine-tuning process was on adjusting the number of epochs. 
In contrast to other studies that typically use fewer than 10 epochs, we selected a significantly larger number, reaching up to 60 epochs for smaller datasets. 
This decision is driven by our specific context: the model is tailored for a single household environment, where task repetition and user-specific details are key. 
Although longer epochs can reduce LLaVA's generalization performance, this trade-off is acceptable for our use case, where memorizing fine-grained details for a single environment is essential. 
We set the Batch Size to 8, Gradient Accumulation to 4, and used BF16 to lower memory usage while maintaining computational precision. 
The training process was conducted within the PEFT framework, using the Cross-Entropy Loss function to guide optimization. 
This approach allowed the model to gradually improve its understanding of visual tasks, fine-tuning its weights with each iteration. 
To address the cold-start problem, when the dataset contained only 3 to 4 samples per task, we employed a strategy of increasing epochs to boost the model’s memory of specific tasks and environments.
Prompt Design and Efficiency: Additionally, we found that long prompts negatively impacted performance, particularly for the LLaVA-7B model. Therefore, we designed concise prompts, such as: 


This prompt structure was selected to align with LLaVA's capabilities, and during inference, we incorporated zero-shot chain-of-thought reasoning, including the prompt ``Let's think step by step'' to enhance task execution. This approach prevents long prompts from degrading the model's reasoning ability while maintaining clarity in task instructions.
As the dataset expanded, we gradually reduced the number of epochs to around 40, ensuring the model could adapt to new tasks without losing its ability to recall past interactions.
A critical focus was placed on explaining key hyperparameters, particularly the number of epochs. 
In contrast to other studies that typically use fewer than 10 epochs, we selected a significantly larger number. 
Smaller epochs are commonly used in scenarios with large datasets and limited computational resources, allowing models to perform multiple updates over shorter training periods to quickly adapt to tasks.
However, in our case, the larger number of epochs (e.g., 40) is well-suited because our model targets a single household environment characterized by task repetition and relatively small datasets. 
By using a large number of epochs, we ensure the model ``memorizes'' specific details without compromising its performance, which is beneficial for long-term adaptation to a specific user.
The training process was conducted using the PEFT framework, which facilitated efficient fine-tuning, particularly for handling the complexity of household tasks.
During the fine-tuning of the LLaVA model with LoRA, the optimization was guided by the Cross-Entropy Loss function. 
This loss function allowed the model to incrementally improve its understanding of visual tasks, adjusting its weights with each training iteration to better adapt to new requirements.
To address the cold-start problem, we adjusted our training strategy when the dataset was small. 
For instance, with only 3 to 4 samples per task, we increased the number of epochs to 60 to enhance the model's memory capacity. 
As the dataset grew, the number of epochs was gradually reduced, ultimately stabilizing at 40 epochs. 
This progressive adjustment ensured a balance between the model’s reasoning abilities and its adaptability.
Thus, even with limited data, the model could generate accurate instructions for visual tasks and quickly adapt to new environments. 


%%%%%%%%%%%%%%%%%%%%%

% To enhance the precision and adaptability of AlignBot, we introduce a memory-based algorithm that prioritizes and selects action plans based on historical interactions.

% Let the database of user feedback be denoted by \( \mathcal{F} = \{ F_1, F_2, \dots, F_N \} \), where each feedback \( F_i \) is associated with a content description \( C_i \) and an initial priority score \( P_i = P_0 \). When the user issues a new task \( I \), the system selects a subset \( S \subset \mathcal{F} \) of feedback entries that are relevant to the task \( I \). Relevance is determined by the similarity \( \text{sim}(C_i, I) \), and the subset \( S \) is defined as follows:

% \[
% S = \{ F_i \mid \text{sim}(C_i, I) > \tau \}
% \]

% where \( \tau \) is a predefined similarity threshold. The feedback entries in \( S \) are then sorted based on their priority scores \( P_i \), resulting in an ordered set \( S_{\text{sorted}} \).

% The priority scores \( P_i \) are dynamically adjusted using a Softmax function to normalize the values, ensuring that all scores remain bounded and introduce a degree of randomness to prevent the system from becoming overly reliant on a limited set of feedback:

% \[
% P_{i_j} = \frac{\exp(\hat{P}_{i_j})}{\sum_{k=1}^{|S|} \exp(\hat{P}_{i_k})}
% \]

% where \( \hat{P}_{i_j} \) represents the unnormalized priority score of feedback \( F_{i_j} \).

% \subsubsection{Adaptive Priority Adjustment}

% To prevent the priority scores from unbounded growth or decay, we incorporate a decaying adjustment mechanism. The adjustment for successful feedback \( F_{i_j} \) is given by:

% \[
% \Delta P_{\text{positive}} = \Delta P_{\text{positive}}^0 \cdot \exp(-\alpha \cdot n_{i_j})
% \]

% Similarly, the adjustment for unsuccessful feedback is:

% \[
% \Delta P_{\text{negative}} = \Delta P_{\text{negative}}^0 \cdot \exp(-\beta \cdot n_{i_j})
% \]

% Here, \( n_{i_j} \) denotes the number of times feedback \( F_{i_j} \) has been used, and \( \alpha \) and \( \beta \) are decay parameters. This ensures that the impact of repeated success or failure diminishes over time, maintaining a balanced approach to priority updating.

% \subsubsection{Weighted Decision-Making}

% In cases where multiple feedback entries are selected, a weighted decision-making process is applied. The final decision \( D \) is computed as a weighted sum of the selected feedback entries:

% \[
% D = \sum_{j=1}^k w_j \cdot F_{i_j}
% \]

% The weights \( w_j \) are determined based on both the priority scores and the confidence levels associated with the feedback:

% \[
% w_j = \frac{P_{i_j} \cdot \text{Confidence}_{i_j}}{\sum_{l=1}^{k} P_{i_l} \cdot \text{Confidence}_{i_l}}
% \]

% This method ensures that more reliable feedback is given greater influence in the final decision, thereby enhancing the robustness of the system.

% \subsubsection{Exploration and Exploitation: \( \epsilon \)-Greedy Strategy}

% To balance the trade-off between exploration of less frequently used feedback and exploitation of proven strategies, we implement an \( \epsilon \) Greedy strategy. This strategy is formalized as follows:

% Given a probability \( \epsilon \) (where \( 0 \leq \epsilon \leq 1 \)), the system selects feedback according to:

% \[
% F_{\text{selected}} =
% \begin{cases}
% F_{\text{random}}, & \text{with probability } \epsilon \\
% F_{\text{max}}, & \text{with probability } 1 - \epsilon
% \end{cases}
% \]

% Here, \( F_{\text{random}} \) is a randomly selected feedback entry from the subset \( S \), promoting exploration. \( F_{\text{max}} \) is the feedback entry with the highest priority score within \( S \), enabling exploitation of the most successful past strategies.

% The parameter \( \epsilon \) controls the balance between exploration and exploitation. A higher \( \epsilon \) increases the likelihood of exploring new feedback, while a lower \( \epsilon \) prioritizes feedback with higher historical success.

% This probabilistic approach ensures that the system does not become overly dependent on a narrow set of strategies, thus maintaining a broader adaptability and preventing stagnation in decision-making processes.

% \subsubsection{Continuous Improvement through Iterative Feedback}

% This algorithm is applied iteratively across multiple task executions. Initially, when all feedback entries have identical scores, a random selection of five feedback entries is made. As tasks are executed, the priority scores are updated based on the success or failure of the generated motion plans. Over time, this process leads to the emergence of a distinct hierarchy among the feedback entries, allowing the system to prioritize the most effective strategies.

% This approach not only refines the system's motion planning capabilities but also adapts to the user's preferences and the specific context of each task. By continuously updating the priority scores and incorporating a balance of exploration and exploitation, the AlignBot model achieves a higher degree of flexibility and precision in its operations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % \subsubsection{Inference Augmented}
% % 大语言模型在推理过程中可能会产生幻觉，导致推理结果错误。为了解决LLaVA的这一问题，我们引入了CoT和Self-Consistency两种方法。CoT方法通过增强prompt，限制模型生成的内容，强化前后文的逻辑关系，从而减少因幻觉导致的逻辑偏差。Self-Consistency方法则通过多次推理，投票选出最常见的答案，降低随机性引发的推理错误。

% % 消融实验结果显示，使用CoT方法后，推理正确率提高了A%；引入Self-Consistency后，正确率同样提高了B%。两种方法结合使用时，正确率提升了C%，有效缓解了幻觉问题对模型准确率的影响。
% Large language models may produce hallucinations during reasoning, leading to incorrect outcomes. To address this issue in LLaVA, we introduced two methods: Chain of Thought (CoT) and Self-Consistency. The CoT method enhances the prompts to constrain the model's generated content and strengthen the logical coherence between contexts, thereby reducing logical errors caused by hallucinations. The Self-Consistency method mitigates errors due to randomness by conducting multiple reasoning iterations and selecting the most frequent answer through a voting process.

% Ablation experiments showed that using the CoT method increased reasoning accuracy by A\%, and the introduction of Self-Consistency also led to a B\% improvement. When both methods were combined, accuracy improved by C\%, effectively mitigating the impact of hallucinations on model accuracy.



% Our AlignBot received high ratings from volunteers due to its excellent performance in real-world use. By combining task descriptions with image context, AlignBot can complete scene-based reminders more effectively. It also does a great job of remembering personalized user preferences, making its responses more accurate and tailored. These strengths make the quality of AlignBot's Cues truly helping users accomplish their tasks.

% AlignBot vs. Finetuned LLaMA2-7b. :As mentioned above, we use LLaMA2-7b instead of llava to generate cues, We examine how effectively a single-modal model can replace LLava in generating cues, comparing its performance against our system. Experiments demonstrate that multi-modal adapters remain crucial. While the finetuned LLaMA2-7B can retain user preferences, its single-modal nature significantly limits its effectiveness. Without image guidance, it can only randomly choose from previously known preferences, making it less accurate in addressing user-specific needs. Moreover, the absence of visual input renders image-based reminders ineffective, as it relies solely on summarizing high-frequency conversations to generate responses. This highlights the inherent shortcomings of a single-modal approach, particularly in tasks requiring visual context and personalized cues.

% AlignBot vs. LLava-7b without Fine-Tuning.: LLaVA1-7B without fine-tuning is significantly limited in its ability to handle tasks involving image-based reasoning. It struggles to accurately identify and interpret objects within a scene, often failing to provide meaningful insights into the status of task-relevant items. Instead, it offers vague, generic descriptions, missing important details that would be critical for task execution. Moreover, the model lacks the capability to infer operational errors from images, which is crucial for guiding robots in real-world environments.  Additionally, without incorporating personalized data, the model cannot tailor its responses to specific user preferences or requirements, making its assistance less relevant and effective in practical scenarios.

% \subsection{Impact of Dataset Size}
% In the third experiment, we investigate the impact of dataset size on the overall success rate of the system. Specifically, we explore how varying the amount of training data affects the performance of LLava, which is responsible for generating cues that are then used by ChatGPT for task planning and execution. We train LLava on datasets of different sizes—200, 500, 800, and 1100 samples—and evaluate how these variations influence the quality of cues and, consequently, the success rate of the tasks performed by ChatGPT. 


% \begin{figure*}[h!]
%     \centering
%     \begin{minipage}[b]{0.24\linewidth}
%         \includegraphics[width=\linewidth, height=2.5cm, keepaspectratio=false]{fig/1.png}
%         \subcaption{Put the apple in fridge}
%     \end{minipage}
%     \begin{minipage}[b]{0.24\linewidth}
%         \includegraphics[width=\linewidth, height=2.5cm, keepaspectratio=false]{fig/2.png}
%         \subcaption{Put all the fruits in the bowl}
%     \end{minipage}
%     \begin{minipage}[b]{0.24\linewidth}
%         \includegraphics[width=\linewidth, height=2.5cm, keepaspectratio=false]{fig/3.png}
%         \subcaption{Heat the potato}
%     \end{minipage}
%     \begin{minipage}[b]{0.24\linewidth}
%         \includegraphics[width=\linewidth, height=2.5cm, keepaspectratio=false]{fig/4.png}
%         \subcaption{Saute carrot slices}
%     \end{minipage}

%     \vspace{0.2cm} % Adds some space between the rows

%     \begin{minipage}[b]{0.24\linewidth}
%         \includegraphics[width=\linewidth, height=2.5cm, keepaspectratio=false]{fig/5.png}
%         \subcaption{Give me some snacks}
%     \end{minipage}
%     \begin{minipage}[b]{0.24\linewidth}
%         \includegraphics[width=\linewidth, height=2.5cm, keepaspectratio=false]{fig/6.png}
%         \subcaption{Organize items}
%     \end{minipage}
%     \begin{minipage}[b]{0.24\linewidth}
%         \includegraphics[width=\linewidth, height=2.5cm, keepaspectratio=false]{fig/7.png}
%         \subcaption{Organize the table}
%     \end{minipage}
%     \begin{minipage}[b]{0.24\linewidth}
%         \includegraphics[width=\linewidth, height=2.5cm, keepaspectratio=false]{fig/8.png}
%         \subcaption{Put things in box}
%     \end{minipage}

%     \caption{Real-world scenarios. We evaluate our AlignBot system in 3 real-world scenarios, encompassing a wide variety of objects and receptacles.}
%     \label{fig:real-world-scenarios}
% \end{figure*}

%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=\linewidth]{fig/test.png}
%    \caption{Real-world objects.}
%    \label{fig:tasks}
%\end{figure} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,references}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \clearpage

% \section*{ACKNOWLEDGMENT}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \onecolumn

% % \section{Appendix}
% % \begin{algorithm}[ht]
% % \caption{Few-Shot Dynamic Retrieval and Priority Update Mechanism}
% % \label{alg:fewshot}
% % \KwIn{
% %     $D = \{p_1, p_2, \dots, p_n\}$: Set of instances with initial priority $f_0 = 0.5$,\\
% %     $t_{\text{new}}$: New task,\\
% %     $S$: Similarity threshold,\\
% %     $\epsilon$: Exploration rate,\\
% %     $\alpha, \beta$: Decay parameters for feedback updates,\\
% %     $\Delta P_{\text{positive}}^0, \Delta P_{\text{negative}}^0$: Initial adjustment values for priority updates.
% % }
% % \KwOut{Updated priority scores for the instances and the weighted decision.}

% % \SetAlgoLined
% % \SetKwFunction{FMain}{run\_iteration}
% % \SetKwFunction{SelectInstances}{select\_instances}
% % \SetKwFunction{UpdatePriority}{update\_priority\_and\_gradient}
% % \SetKwFunction{Softmax}{softmax}
% % \SetKwFunction{SimulateSimilarity}{simulate\_similarity}
% % \SetKwFunction{WeightedDecision}{weighted\_decision}

% % \textbf{Initialization:} Set initial priorities $f_i = f_0$, gradients $g_i = 0$, and use count $n_i = 0$ for all instances.\\

% % \While{new task $t_{\text{new}}$ arrives}{
% %     \tcc{Instance Selection}
% %     Compute similarity $sim(t_i, t_{\text{new}})$ for each instance $p_i \in D$ using TF-IDF and cosine similarity.\\
% %     Select a subset $D_r'$ such that $sim(t_i, t_{\text{new}}) > S$. If fewer than required, select additional random instances.\\

% %     Apply an $\epsilon$-Greedy strategy:
% %     \If{random value $< \epsilon$}{
% %         Select random instances from $D_r'$. 
% %     }
% %     \Else{
% %         Normalize priorities with the Softmax function:
% %         \[
% %         f_{i_j} = \frac{\exp(f_{i_j})}{\sum_{k} \exp(f_{i_k})}
% %         \]
% %         Sort instances by normalized priority and select top-k.\\
% %     }

% %     \tcc{Priority and Gradient Update}
% %     For each selected instance $p_i$:
% %     \If{$p_i$ was useful}{
% %         Update gradient $g_i$:
% %         \[
% %         g_i = g_i + \Delta P_{\text{positive}}^0 \cdot \exp(-\alpha \cdot n_i)
% %         \]
% %     }
% %     \Else{
% %         Update gradient $g_i$:
% %         \[
% %         g_i = g_i - \Delta P_{\text{negative}}^0 \cdot \exp(-\beta \cdot n_i)
% %         \]
% %     }
% %     Update priority $f_i$ based on gradient:
% %     \[
% %     f_i = \min(\max(0.1, f_i + g_i), 1.0)
% %     \]
% %     Increment $n_i$ by 1.

% %     \tcc{Weighted Decision}
% %     Compute the weighted decision $D$ based on priority and confidence levels:
% %     \[
% %     D = \sum_{i=1}^{k} \frac{f_i \cdot \text{Confidence}_i}{\sum_{l=1}^{k} f_l \cdot \text{Confidence}_l}
% %     \]
% % }

% % \end{algorithm}
% GPT-4o Prompt:

% \noindent
% \begin{minipage}[\textheight]{\textwidth}
% \lstset{
%     basicstyle=\ttfamily\small,
%     breaklines=true,
%     breakatwhitespace=false,
%     columns=fullflexible,
%     keepspaces=true,
%     showspaces=false,
%     showstringspaces=false,
%     tabsize=4
% }

% \begin{lstlisting}
%   You are controlling a one-armed robot.

%   **Task Objective:**
%   Your task is to complete the following goal:
%   {goal}

%   **Current Environment:**
%   Please analyze the image carefully, ensuring that all objects, particularly those relevant to the goal, are identified and accounted for.

%   **Past Successes:**
%   Refer to these past successful cases relevant to the current goal:
%   {Successes}
%   Note that these Successful cases generated in the past may not be applicable to the current situation.
    
%   **cues:**
%   You need to pay careful attention to the following cues:
%   {cues}

%   **User Feedback:**
%   These are the plans you generated in the previous rounds, and the user provided feedback for these plans:
%   {records}
%   You need to pay special attention to user feedback to make sure you don’t make the same mistakes.
  
%   **Available Actions:**
%   Here are the all actions you can use to achieve the goal:
%   - **turnright**: Rotate the robotic arm to the right.
%   - **turnleft**: Rotate the robotic arm to the left.
%   - **walkforward**: Advance the robotic arm forward.
%   - **walktowards <obj>**: Move the robotic arm towards the specified object.
%   - **moveto <x, y, z>**: Navigate to coordinates x, y, z.
%   - **grab <obj>**: Grasp the specified object. Release any held item before grabbing a new one.
%   - **switchon <obj>**: Activate the specified object.
%   - **switchoff <obj>**: Deactivate the specified object.
%   - **open <obj>**: Open the specified object.
%   - **close <obj>**: Close the specified object.
%   - **lookat <obj>**: Focus on the specified object.
%   - **find <obj>**: Locate the specified object.
%   - **turnto <obj>**: Orient towards the specified object.
%   - **pointat <obj>**: Point to the specified object.
%   - **putin <obj1> <obj2>**: Place the first object into the second.
%   - **puton <obj1> <obj2>**: Place the first object on top of the second.
%   - **putback <obj1> <obj2>**: Return the first object into the second.
%   - **push <obj>**: Push the specified object.
%   - **pull <obj>**: Pull the specified object.
%   - **rotate <obj>**: Rotate the specified object.
%   - **tilt <obj>**: Tilt the specified object.
%   - **cut <obj>**: Cut the specified object.
%   - **flip <obj>**: Flip the specified object.
%   - **wait <n>**: Pause for n minutes.
%   - **done**: Signal task completion.

%   **Output Structure:**
%   - Formulate a step-by-step action plan using only the actions listed above.
%   - Each step should adhere to the following syntax:
%       '''
%       [action] ("object1", (optional: "object2"))
%       '''
%   - Conclude the plan with the **done** action.
%   - In the action plan, briefly describe the color and shape of the object

%   **Example:**
%   For the goal "Put the fork into the cup":
%       '''
%       def Put_the_fork_into_the_cup():
%       find ("grey fork")
%       walktowards ("grey fork")
%       grab ("grey fork")
%       find ("red cup")
%       putin ("grey fork", "red cup")
%       done
%       '''
% \end{lstlisting}
% \end{minipage}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \onecolumn

% \section{Appendix}

% LLava Prompt:

% \noindent
% \begin{minipage}[\textheight]{\textwidth}
% \lstset{
%     basicstyle=\ttfamily\small,
%     breaklines=true,
%     breakatwhitespace=false,
%     columns=fullflexible,
%     keepspaces=true,
%     showspaces=false,
%     showstringspaces=false,
%     tabsize=4
% }

% \begin{lstlisting}
%   You are a multimodal large language model that processes images and instructions. 
  
%   **Task Objective:**
%   {User} want robot to {goal}.
%   Your task is to provide step-by-step cues to the robot to complete the goals given by the user. The cues should be detailed, reflecting user-specific information and the current scene. 

%   Follow these guidelines:
%   1. **Personalized cues:**
%     - Generate cues based on user
%     - Include user preferences and specific rules for item placement.
%     - Mention any habitual actions the user typically follows.

%   2. **Scene cues:**
%     - Generate cues based on picture and goal
%     - Describe all items visible in the image, including their status, position, and any notable details.
%     - Reference any past successful scenarios or considerations similar to the current scene.

%   3. **Step-by-Step Action cues:**
%     - Generate cues based on picture and goal
%     - Provide a detailed, step-by-step cue for each action, ensuring clarity and precision.
%     - Consider the robot’s single-arm constraint: remind that only one action can be performed at a time.
%     - Include any specific instructions related to the current scene and the user's preferences.

%   **Output Structure:**
%   1. **User Preferences:**
%     - [Include relevant personalized information based on the user’s habits or rules.]

%   2. **Scene Description:**
%     - [Provide a detailed description of the items and their status in the image.]

%   3. **Step-by-Step Action cues:**
%     - cue 1: [Detailed cue for the first action, considering robot’s single-arm constraint.]
%     - cue 2: [Next detailed cue.]
%     - ...
%     - Final cue: [Final detailed cue, ensuring all tasks are completed according to the user’s preferences and scene specifics.]

%   **Few-Shot Examples:**

%   Example 1:
%   - Carefully identify the objects on the table in the picture and put them into the drawers. 
%   - Put drinks in drawer 1. 
%   - Put kitchen utensils in drawer 3. The kitchen utensils in the picture are a white tray and a kitchen knife. Put them in drawer 3.
%   - The yellow item is actually a tea beverage. You should open drawer 1 before grabbing things.

%   Example 2:
%   - Put snacks in drawer 2 and kitchen utensils in drawer 3.
%   - The kitchen utensils in the picture are a cutting board and a fruit knife.
%   - The pink fruit knife is on the cutting board. Put them into drawer 3. You should open drawer 3 before grabbing things.

%   Example 3:
%   - Put drinks in drawer 1.
%   - Drawer 1 is already open. You do not need to open it again. Close drawer 1 at the end.

%   Ensure each cue is clear, follows the constraints, and aligns with the user's preferences and the scene description.
% \end{lstlisting}
% \end{minipage}
\end{document}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 在测试中，我们比较了llava 7b和llava 13b
% llava 7b 的推理能力和图像识别能力非常有限但是数据需求量小，
% 13b的推理能力和图像识别能力提升，但是少量的数据非常难影响模型

% 我们的数据有三个特点：1.数据量少，每个任务也就50-100个场景 2.任务多且任务环境较为复杂，有处于不同状态的物品，还有非常多的干扰物 3.有不同的用户

% 因此我们需要模型能够在有限数据下快速记忆，这也是增大epoch的主要原因
% 与之相配合的是
% 1.llava的prompt不能太长。llava 7b 无法理解长prompt。最好是直接以对话的形式调用llava。因此选择<User ID> wants robot to <Task Description>. Can you provide some reminders to robot? 这样的模式
% 2.数据集中的userfeedback也要处理修整，使用简洁的语句。对于相同的物品状态或环境特点尽量使用同样的指导句子。在复杂场景中直接用这些指导句子排列组合来描述

% 此外为了在有限数据量下增强llava图像识别能力，使其快速熟悉当前家庭环境，增加了两个小数据集来让llava捕捉细粒度的视觉细节

% Batch Size & Gradient Accumulation设置为8和4，Data Type: BF16  这主要是为了降低显存占用量，同时保持计算精度，

% semantic grouding和cue generation的训练过程是在semantic grouding训练后的checkpoint上继续训练cue generation
% 这样的设计主要是认为cue generation需要用到semantic grouding任务阶段学到的知识，因此分阶段训练能够有所继承。并且两个任务的目标不太一样，通过分阶段训练可以避免它们之间的负面干扰


% 此外还有一个点为什么选择多模态模型
% 1.chatgpt每次plan失败的原因各不相同，并且与任务发生场景高度相关。也就是说user的feedback也会更具场景不同而不同，这些不同难以通过文字进行简要概述并区分
% 2.chatgpt非常容易被误导。例如即使chatgpt能够识别图像中的冰箱开着，但是直接告知他冰箱关着，他就会以冰箱关着为准。因此准确的基于图像的提醒是重要的


% \begin{table}[H]
% \centering
% \caption{Common tasks}
% \begin{tabular}{c|c}
% \toprule
%     Method & Success Rate\\
%     \midrule
%     GPT4o only & 22.59\%  \\
%     \midrule
%     GPT4o with memory base & 25.92\%\\
%     \midrule
%     LLaMA2-7b with GPT4o & 23.71\%\\
%     \midrule
%     AlignBot & 84.81\%\\
%     \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[H]
% \centering
% \caption{Personalized task}
% \begin{tabular}{c|c}
% \toprule
%     Method & Success Rate\\
%     \midrule
%     GPT4o only & 12.96\%  \\
%     \midrule
%     GPT4o with memory base & 40.37\%\\
%     \midrule
%     LLaMA2-7b with GPT4o & 56.67\%\\
%     \midrule
%     AlignBot & 88.89\%\\
%     \bottomrule
% \end{tabular}
% \end{table}

% \begin{table*}[h!]
% \centering
% \caption{Success Rate of common tasks}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{cccccccccc}
% \toprule
%     Method & put apple in fridge & boil water & cut carrot & heat pot & heat potato & put apple in bowl & put fruits in bowl & put pear in Drawer & Saute carrot slices\\
%     \midrule
%     GPT4o only & 0\% & 13.3\% & 36.7\% & 46.7\% & 3.3\% & 40\% & 56.7\% & 0\% & 6.7\%\\
%     \midrule
%     GPT4o with memory base & 33.3\% & 26.7\% & 40\% & 16.7\% & 13.3\% & 36.7\% & 46.7\% & 6.7\% & 13.3\%\\
%     \midrule
%     LLaMA2-7b with GPT4o & 13.3\% & 13.3\% & 3.3\% & 3.3\% & 10\% & 40\% & 6.7\% & 20\% & 20\%\\
%     \midrule
%     AlignBot & 90\% & 83.3\% & 96.7\% & 96.7\% & 80\% & 93.3\% & 73.3\% & 93.3\% & 56.7\%\\
%     \bottomrule
% \end{tabular}}
% \label{task1}
% \end{table*}

% \begin{table*}[h!]
% \centering
% \caption{Success Rate of personalized tasks}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{cccccccccc}
% \toprule
%     Method & Organize items & put things in drawer & give something to drink & give snacks & give cup & give sugar & give vinegar & Organize table & put things in box\\
%     \midrule
%     GPT4o only & 0\% & 0\% & 30\% & 33.3\% & 30\% & 3.3\% & 20\% & 0\% & 0\%\\
%     \midrule
%     GPT4o with memory base & 10\% & 3.3\% & 40\% & 36.7\% & 43.4\% & 80\% & 83.3\% & 40\% & 26.7\%\\
%     \midrule
%     LLaMA2-7b with GPT4o & 3.3\% & 6.7\% & 56.7\% & 40\% & 96.7\% & 96.7\% & 93.3\% & 43.4\% & 80\%\\
%     \midrule
%     AlignBot & 70\% & 76.7\% & 96.7\% & 90\% & 96.7\% & 96.7\% & 96.7\% & 86.7\% & 93.3\%\\
%     \bottomrule
% \end{tabular}}
% \label{task2}
% \end{table*}
% From Table~\ref{task1} and \ref{task2} we can see that compared to other methods, our AlignBot shows better performance than the baseline on every task. AlignBot effectively remembers user preferences and incorporates them into the decision-making process. In addition, it is also good at accurately monitoring the status and arrangement of items in the current scene and making reasonable adjustments in planning, which helps AlignBot avoid unnecessary steps and logic errors.

% AlignBot vs. GPT4o: In common tasks, gpt4o has very poor spatial understanding. It cannot recognize whether there are obstacles above the target object. It cannot recognize the status and position of some items, such as whether a drawer is open or closed or whether a pot is on the stove. It also cannot understand the single-arm structure of the robot, and often sets the robot to operate other targets while grasping objects in planning. In personalized tasks, due to lack of information, gpt4o will randomly select the target object in the picture. For ambiguous commands such as Organize items, gpt4o will randomly plan based on some common sense understanding. This result proves the effectiveness and correctness of our method, which is to build a database based on user feedback and create an adapter for GPT-4o powered on the database.

% AlignBot vs. GPT-4o with Memory: Even with the help of the database, the success rate of planning by GPT-4o is much lower than that of our method. This is because user feedback is based on scenarios, and different scenarios require different states and locations of items to be noted. Incorrect reminders not only fail to improve planning, but also mislead GPT4o, making it unable to correctly identify image information. In addition, too much information increases the difficulty of LLM in filtering information. This result verifies the importance of building an adapter that can generate correct reminders based on the scenario.
 
% AlignBot vs. Finetuned LLaMA2-7b with GPT4o: Finetuned LLaMA2-7b remembers the user's preferences and can give reminders based on the user's tendencies. And it can correct some high-frequency planning step errors. However, due to the absence of explicit scene guidance and spatial awareness, the finetuned LLaMA2-7b model struggles to provide accurate information about the status or arrangement of items in the environment. This makes reminders less reliable and even misleading. This proves that multi-modal adapters are very necessary.



% \begin{table}[h!]
% \centering
% \caption{Rating guidelines for human raters in the experiments.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{p{0.1\linewidth} p{0.8\linewidth}}
% \toprule
%     Points & Rating Guidelines\\
%     \midrule
%     0 & Cues are so irrelevant to the scene that it has no corrective effect at all.\\
%     \midrule
%     1 & Although there are some errors, cues contain partially correct item status reminders, personalized reminders, or planning step reminders.\\
%     \midrule
%     2 & There are no errors, but cues only contain partially correct item status reminders, personalized reminders or planning step reminders.\\
%     \midrule
%     3 & Cues accurately includes item status reminders, personalized reminders and planning step reminders.\\
%     \bottomrule
% \end{tabular}}
% \end{table}


% \begin{itemize}
%     \item put the apple in fridge
%     \item boil water
%     \item cut carrot
%     \item heat the pot
%     \item heat the potato
%     \item put the apple in bowl
%     \item put all the fruits in the bowl
%     \item put pear in the Drawer
%     \item Saute carrot slices
%     \item Organize items
%     \item put things in drawer
%     \item give me something to drink
%     \item give me some snacks
%     \item give me my cup 
%     \item give me salt
%     \item give me sugar
%     \item give me vinegar 
%     \item give me soy sauce
%     \item put things in box
%     \item Organize the table
% \end{itemize}


% Personalization is considered in three main directions:
% \begin{itemize} 
% \item Scene Personalization: This direction focuses on the specific scene settings of each household, such as fixed storage rules and organization patterns. 
% \item User Preference Personalization: This direction emphasizes each user’s personal preferences and historical behaviors, such as favorite snacks or frequently used cups. 
% \item Item Personalization: This direction considers the special cultural background or unique item usage habits within the family. 
% \end{itemize}


% For all our real-world manipulation experiments, we use a UFactory XArm 6 robot. It is a versatile 6-degree-of-freedom manipulator with a $700 mm$ reach, $5 kg$ payload, $± 0.1 mm$ repeatability, and $1000 mm/s$ maximum speed. It also supports multiple modes of motion control, such as joint position control and velocity control that can be seamlessly adapted to our system. We use XArm gripper with adapted UMI compliant fingers. The arm is rigidly mounted on a mobile base to easily change to different scenes. However, we assume it is a fixed-based arm rather than a mobile manipulator. We use \textit{xArm-Python-SDK} to control the robot.

% The robot is equipped with two Intel RealSense D435i cameras. One mounted on the wrist and another on the shoulder. We use the \textit{pyrealsense2} package to communicate with the camera. We use two RGB images with a size of $640\times480$ pixels and a framerate of $60 Hz$. Additionally, for the hand camera, we use stereo infrared images with a size of $848\times480$ pixels and a framerate of $90 Hz$.

% We initially positioned the end-effector approximately $200 cm$ away from the object. The task space, where the objects were placed, was defined to ensure that the object was always at least partially visible in the image from the end-effector's initial pose.

% \yan{
    % task-relvant case: 无
    % cues: 无
    % }
    % \yan{
    % task-relvant case: 相同task下，随机选择，可能面临对应不上，可能缺失，或者没有用。
    % cues: 相同task下，随机选择，可能面临对应不上，可能缺失，或者没有用。
    % }
    % \yan{
    % task-relvant case: 一样的， 动态（？）
    % cues: 单模态。但是可能对于不不需要视觉的personalized的任务会比较有效果。
    % }


    
% , as shown below:
% \begin{quote}
% \emph{Q: \textless User ID\textgreater wants robot to \textless Task Description\textgreater. Can you provide some reminders to robot?\\
% A: \textless Instruction-format cues provided users\textgreater.}
% \end{quote}
